Don't Stop Pretraining: Adapt Language Models to Domains and Tasks

Language models pretrained on text from a wide variety of sources form the foundation of today's NLP. In light of the success of these broad-coverage models, we investigate whether it is still helpful to tailor a pretrained model to the domain of a target task. We present a study across four domains (biomedical and computer science publications, news, and reviews) and eight classification tasks, showing that a second phase of pretraining in-domain (domain-adaptive pretraining) leads to performance gains, under both high- and low-resource settings. Moreover, adapting to the task's unlabeled data (task-adaptive pretraining) improves performance even after domain-adaptive pretraining. Finally, we show that adapting to a task corpus augmented using simple data selection strategies is an effective alternative, especially when resources for domain-adaptive pretraining might be unavailable. Overall, we consistently find that multi-phase adaptive pretraining offers large gains in task performance.

==> archived/2_background.tex <==
\section{Background: Pretraining}
\label{sec:roberta}

% \todo{define pretraining, and then proceed to explain how \roberta was pretrained, and the domain- and task- adaptive settings.}

%\subsection{\roberta}

\roberta follows the same architecture as its predecessor \bert \cite{devlin-etal-2019-bert} but is trained only with the masked language modeling training objective (i.e., cross-entropy loss on predicting randomly masked tokens) and on substantially more data. 
In particular, over 160 GB of uncompressed raw text from different English-language corpora was used, see Appendix \sect{sec:roberta_pretraining} for details. 
The pre-processed corpora was not released, but could potentially be replicated with considerable effort using the provided instructions for each corpus. %(see footnotes 2--6).{\todo{Check footnote numbers in the final version.}}

The key assumption behind using a large pretraining corpus was that given enough data to train on, the representations from these models are general enough to be applicable for high performance across a variety of tasks in English.
Our work questions this fundamental assumption.


In the next two sections, we investigate the benefits of continued pretraining of \roberta to two types of unlabeled data: (i) large corpora of domain-specific text \sect{sec:dapt}, and (ii) available unlabeled data of a given task \sect{sec:tapt}. 
% We continue pretraining instead of training from scratch to preserve already acquired knowledge of the original domains while adapting to new domains.
% Moreover, this makes the pretraining step more efficient, as the language model takes fewer iterations to reach convergence \todo{This is not exactly clear.}.
% After pretraining, all \roberta models are normally fine-tuned with the labeled training data. 


==> archived/3_dapt.tex <==
\input{tables/exp_mlm.tex}

\section{\daptfull}
\label{sec:dapt}

We investigate four domains for adaptation, namely biomedical journal, computer science (CS) publications, newstext from \realnews \citep{zellers2019defending} and \amazon.
Based on our prior knowledge of the training corpora for \roberta, we hypothesize that with the exception of news, all other domains are relatively new for \roberta.
However, we choose to investigate the news domain specifically to answer whether there are additional benefits of exposure to even more news data.
We continue pretraining \roberta on a large corpus of unlabeled domain-specific text for each of the four domains, resulting in four domain-adapted language models. 
Table \ref{tab:domain_datasets} lists the specifics of unlabeled datasets in the four domains.

% \paragraph{Domain datasets} 
% We experiment with four domains: biomedical papers, computer science papers, news articles, and Amazon reviews. 
% The details of domain-specific datasets are given in Table \ref{tab:domain_datasets}. 


\paragraph{Domain shift} 

We posit that \roberta's masked language modeling (MLM) loss could serve as an indicator of the similarity of its domain\footnote{Specifically, the different domains on which \roberta was trained, described in Appendix \ref{sec:roberta_pretraining}.} to different target domains.
Towards this end, we compute \roberta's test MLM loss calculated on 50K randomly selected documents of news articles, Amazon reviews, biomedical, and computer science publications.\footnote{We mask tokens with the probability of $0.15$ for computing this loss, following the default recommendation.} 
As a baseline, we randomly sample 50K documents from sources similar to \roberta's own pretraining corpus (see Appendix \sect{sec:roberta_pretraining} for details\footnote{Instead of \textsc{CC-News}, we used \textsc{RealNews} which has a similar data distribution. We did not sample from \textsc{OpenWebText}.}).
% We replicated \todo{Arman did. Can we say this?} a portion of \textsc{RoBERTa}s pretraining corpus 
% that consist of \textsc{Wikipedia}, \textsc{BookCorpus}, \textsc{RealNews}, and \textsc{STORIES} (see \sect{sec:roberta} for details). 

Our results in Table \ref{tab:domain_shift} align with the intuition that test loss will be comparable to the baseline for domains closer to the ones in \roberta's training corpus. 
Indeed, we see that news articles present the least amount of domain novelty, whereas articles from biomedicine, computer science and reviews are farther away.
The relatively higher loss for the latter domains suggests that tasks in these domains could benefit from exposure to the target domain. 
This simple strategy could potentially serve as an indicator of whether a rather expensive domain-adaptive pretraining is valuable for the domain of interest.




% , although \roberta's pretraining corpus is seemingly diverse enough \swabha{not sure if this is a claim they made or we are making?} to address most of the variation in English language. 

\input{tables/data_domains.tex}

==> archived/4_tapt.tex <==
\section{\taptfull}
\label{sec:tapt}

\input{tables/data_tasks}

A single NLP task often focuses on only a small subset of its broader domain.  Often, the training and test corpora for a task are carefully curated to capture a niche of language that is rich in a phenomena of interest.
As an example, the \chemprot task in our experiments is aimed at automatically extracting relationships between chemical compounds and proteins. Its training and test corpora consist of abstracts from chemistry-related papers---a small fraction of the broader domain of all medical text.  In fact, the selection criteria for the CHEMDNER corpus used in \chemprot restricts the data in a variety of specific ways: it includes only abstracts of articles from hand-selected categories of PubMed journals with high impact factor, published in recent years \cite{krallinger2015chemdner}.  In such cases where the task data is a narrowly-defined subset of the domain, pretraining on it directly or on similar task-relevant data may be helpful.

{\em \taptfull} (\tapt), which we use to denote pretraining on the unlabeled training set for a given task, has been shown to be effective in previous work \cite{howard-ruder-2018-universal}.  
Compared to domain-adaptive pretraining, the task-adaptive approach strikes a different trade-off: it uses a far smaller pretraining corpus, but one that is much more task-relevant.
%, and show that the task-adaptive approach improves performance with or without domain-adaptive pretraining, and can be more computationally efficient, but provides less benefit when transferring across tasks.
We distinguish between two types of task-adaptive pretraining.  
One, the {\em micro} setting, is when the pretraining corpus is exactly the labeled training data for the task, with the labels removed.  
This corresponds to the setting studied in previous work.  
The other, the {\em macro} setting, is when we have a larger unlabeled task-relevant training set, and a smaller labeled training set.
The macro setting is often applicable in practice, since it is typically cheap to acquire relevant unlabeled examples for a task, but expensive to label them.

%\todo{Task dataset in our study are a "focused subset" of a single domain. We will never be able to train on all the medical data. Cite ULMFit's motivation for task-adaptive pretraining. Trade-off between data and how much task-focused the data is. Domain vs task: they complement each other, transferability, cost of training... Task-adaptive is always good. Granularity.}

%We wonder \swabha{how? do you mean investigate?} if the variation of the language in a dataset of a particular task is subsumed in %whatever is considered to be target domain for that dataset. 
%If that is the case, additional pretraining on available unlabeled data of a given task (task-adaptive pretraining) after domain-adaptive %pretraining will not improve task performance. 
%Otherwise, we wonder can we replace domain-adaptive pretraining with task-adaptive pretraining. 
%For each out of eight task datasets we continue pretraining both the original \roberta and the corresponding domain-adapted \roberta on the training data of a task. 
%See Table \ref{tab:task_datasets} for a list of the tasks and their datasets.

\paragraph{Task datasets} 

We consider two classification tasks in each of four domains.  
The details of these tasks and their datasets are given in Table \ref{tab:data_tasks}.  
We note that, following previous work \cite{Beltagy2019SciBERTAP}, we treat relation extraction as a text classification problem. 
To simulate a setting in which we have large amounts of curated data for macro task-adaptive fine-tuning in the medical domain, we downsample the training data of the \rct dataset to 500 examples, and treat the rest of the training data as unlabeled. 
% Because the \hp dataset does not have a publicly available test set, we report only dev set numbers on this task. \swabha{this is incorrect!}

% \paragraph{Train/dev/test splits} \todo{Suchin: fill in the following information.} 
% \swabha{Commented the above, do not need a new paragraph to talk about t/d/t splits.}
% \todo{How did we decide which datasets to down-sample for a low-resource study? }

==> archived/5_experimental_setup.tex <==
\subsection{Experimental Setup}
\label{sec:training}

\paragraph{Pre-Processing}
The unlabeled corpora in each domain was pre-processed prior to language model training.
Abstracts and body paragraphs from biomedical and computer science articles were used after sentence splitting using \texttt{ScispaCy} \citep{Neumann_2019}.  
We used summaries and full text of each news article, and the entire body of review from Amazon reviews.
For both news and reviews, we perform sentence splitting using \texttt{spaCy} \citep{spacy2}.

For all pretraining corpora, we follow \citet{Liu2019RoBERTaAR} in constructing input sequences as chains of contiguous sentences that do not cross document boundaries.  Long sequences are truncated randomly at the beginning or end to 512 tokens.

\paragraph{Domain- and Task- Adaptive Pretraining}
Our language model adaptation follows the settings prescribed for training \roberta in \citet{Liu2019RoBERTaAR}. 
We report all hyperparameters used for adaptive pretraining in  Appendix \sect{sec:hyperparam_appendix}. 
% For domain-adaptive pretraining, we train \roberta on each domain for 12.5K steps \suchin{confirm this number with kyle} 
% \kyle{confirmed; add details:  
We used the Adam optimizer \cite{kingma2014adam}, a linear learning rate scheduler with $6$\% warm-up, a maximum learning rate of $0.0005$ and effective batch size of $2048$ through gradient accumulation, as recommended in \citet{Liu2019RoBERTaAR}.
Each model was pretrained on its own v3-8 TPU for one week.  
Our implementation uses the \texttt{HuggingFace Transformers} library \citep{wolf2019huggingfaces}\footnote{\url{https://github.com/huggingface/transformers}} and \texttt{PyTorch XLA} for TPU compatibility\footnote{\url{https://github.com/pytorch/xla}}. 

We artificially augmented each dataset for \tapt \ana{The abbreviation introduced here for the first time without explicitly saying this is task-adaptive pretraining.} \swabha{Nope it's also in the intro and section 4 now.}by randomly masking different tokens across epochs.
Each dataset was trained on for 100 epochs. 
For tasks with less than 5K examples, we used a batch size of 256. \swabha{BS, epoch etc. are too low level, can be moved to appendix?}
Each adaptive pretraining experiment was performed on a single v3-8 TPU from Google Cloud \footnote{\url{http://github.com/allenai/tpu-pretrain}}. We will release our adapted \roberta models\footnote{\url{https://anonymous}}.

% We use a batch size of 2048 and the maximum sequence length of 512 word pieces. 
% We use the AdamW optimizer, with a learning rate of \todo{?}. 
% We train for \todo{?} epochs, checkpointing the model after each epoch. 

\paragraph{Downstream Tasks}
We perform supervised fine-tuning of \roberta for all downstream classification tasks. 
All hyperparameters used in these experiments are reported in Appendix \sect{sec:hyperparam_appendix}. 

We use an early stopping criterion based on validation performance. 
The only exception is \hp, which does not have a publicly available development or test set. 
For this task, we perform five-fold jack-knifing \todo{CITE}, with an $80/20$ split for train/test.
We report the average performance across the five different test splits.

For all experiments, we report the mean and standard deviation of the performance across five randomly chosen seeds. 
We report macro-$F_1$ test scores for all tasks except \chemprot, for which we use micro-$F_1$, following previous work on this task. 
Our classifiers are implemented using the \texttt{AllenNLP} \cite{gardner2018allennlp} library, and our code will be made publicly available \footnote{\url{https://anonymous}}. 

==> archived/5_transfer.tex <==

\section{Transfer among Domains and Tasks}
\label{sec:transfer-results}


In Section \sect{sec:dapt}, we found that domain-adapted LMs generalize better to tasks within the said domain, compared to the \roberta LM.
This is especially true when the target domain is distant from the source domain(s) of \roberta. 
We also found that adaptation to a supposedly distant domain (i.e., \realnews) can improve performance of an end-task in a given domain (i.e., \imdb).
\swabha{Isn't this claim subject to change with the new reviews LM?}
To understand this finding better, we provide some qualitative analysis (\sect{sec:cd_transfer}).
We will also investigate transfer of task-adapted LMs to other tasks in the same domain (\sect{sec:ct_transfer}). 



==> archived/exp_dt_apt.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}cc|cccccccc@{}}
\toprule
\multicolumn{2}{c|}{Pretraining}  
& \multicolumn{2}{c}{\med}          
& \multicolumn{2}{c}{\cs}              
& \multicolumn{2}{c}{\realnews}  
& \multicolumn{2}{c}{\amazon}      \\
 \cline{1-2} \cline{3-4} \cline{5-6} \cline{7-8} \cline{9-10} 
Phase II & Phase III & \chemprot         & \rct          & \arccite     & \sciie        & \hp & \ag$^\dagger$      & \helpful$^\dagger$  & \imdb$^\dagger$        \\
\midrule
-      & -    & $81.5_{1.1}$ & $71.5_{1.1}$ & $64.8_{3.6}$ & $78.9_{1.6}$ & $82.9_{1.6}$ & $93.5_{0.4}$ & $61.4_{2.7}$ & $92.3_{0.5}$ \\
DAPT & -    & $83.0_{0.7}$ & $74.9_{0.6}$ & $71.1_{4.5}$ & $79.8_{1.2}$ & $82.7_{2.2}$ & $93.6_{0.2}$ & $65.6_{2.2}$ & $93.2_{0.5}$ \\
TAPT   & -    & $82.0_{0.2}$ & $72.9_{0.4}$ & $68.3_{4.0}$ & $79.6_{1.5}$ & \boldmath{$83.9_{2.6}$} & $94.0_{0.2}$ & $69.8_{3.0}$ & $92.5_{0.3}$ \\
DAPT & TAPT & \boldmath{$84.8_{0.5}$} & \boldmath{$76.0_{0.7}$} & \boldmath{$77.5_{3.1}$} & \boldmath{$80.2_{1.5}$} & $83.8_{2.6}$ &     \boldmath{$94.2_{0.1}$}       & \boldmath{$69.9_{2.1}$} & \boldmath{$95.3_{0.1}$} \\
\midrule[0.03em]
$\lnot$ DAPT & - & $80.6_{1.2}$ & $72.7_{0.7}$ & $67.7_{5.7}$ & $80.0_{3.0}$ & $79.0_{4.1}$ &  $93.4_{0.2}$ & $66.9_{3.2}$ & $94.5_{0.3}$& 
\bottomrule
\end{tabular}}
\caption{Results on different phases of adaptive pretraining. 
Phase I is the baseline \roberta pretraining (Row 1), which we compare with \dapt (Row 2), \tapt (Row 3), and a combination of both (Row 4).
$\dagger$ indicates high-resource settings.
All results are test macro-$F_1$, except for \chemprot, for which we report micro-$F_1$. 
% For \hp, we report test set performance under a five-fold jackknife.  
The last row describes a baseline pretraining without accounting for the domain of interest. 
\todo{Repeat Helpfulness and IMDB with a newer reviews-\roberta (DAPT, DAPT + TAPT, DAPT+oracle-TAPT, transferability).}}
\label{tab:main}
\end{table*}

==> archived/exp_mlm.tex <==
\begin{table}[t]
\centering
\resizebox{0.85\columnwidth}{!}{
\begin{tabular}{lr}
\toprule
\textbf{Domain} & \textbf{MLM Test-Loss}\\ 
\midrule
\med
& $1.85$ \\
\cs
& $2.30$   \\
\realnews 
& $1.51$  \\
\amazon  
& $2.40$  \\
\midrule
\roberta (Baseline) 
& $1.66$\\
\bottomrule
\end{tabular}}
\caption{
\roberta's masked LM loss on $50$K randomly sampled held-out documents from each domain. 
The baseline performance is on data sampled from sources similar to \roberta's pretraining corpus. \swabha{Replace with a bar chart?}
} 
\label{tab:domain_shift}
\end{table}

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{Computational Requirements}

\paragraph{Do domain-adapted \textsc{RoBERTa}s suffer from catastrophic forgetting?}
Catastrophic forgetting is a widely reported phenomena in neural models of language \cite{}.
We experimented with \suchin{Given the lack of interesting results here, I would suggest we wrap any discussion of "forgetting" into "transferability" of adapted RoBERTas.}

\paragraph{How to measure domain shift?} In practice, we want to know whether domain-adaptive pretraining will be useful before spending resources on another round of pretraining. It is appealing to use the masked LM (MLM) loss as an indicator of usefulness of domain-adaptive pretraining. However, the reasons why the MLM loss is high could be because the domain is out-of-domain for a language model, or because the domain is just more difficult to the model. An alternative to the MLM loss is to compare n-gram statistics of a target domain and pretraining corpus. Unfortunately, this is generally not straightforward since it requires replicating a massive pertaining corpus which is also time and resource consuming. We show that tasks in domains for which \roberta's test MLM loss is higher than the loss on a sample of the original pretraining corpus (see Table \ref{tab:domain_shift}), indeed benefit from domain-adaptive pretraining (see Table \ref{tab:main_test_results}, row 1--2), and other way around. This might be a useful heuristic in practice, but in future work, we want to investigate a more robust measure that distinguishes the domain shift from text complexity for a given language model.   

==> tables/3_masked_lm_study.tex <==
\begin{table}[t]
\small
\centering
{
\begin{tabular}{lccccc}
\toprule
%  & \multicolumn{5}{c}{}\\
%  \cmidrule{2-6} 
 & PT & \med & \cs & \news & \reviews \\
\midrule
%$\mathcal{L}_{\roberta}$ 
\textsc{RoBa.} & 1.19 & 1.32 & 1.63 & 1.08 & 2.10 \\
%$\mathcal{L}_{\dapt}$ 
\dapt& - & 0.99 & 1.34 & 1.16 & 1.93 \\
\midrule
\makecell[c]{$\Delta$} & - &  0.33 & 0.29 & --0.08 & 0.17 \\
% \makecell[c]{$\Delta\widetilde{\mathcal{L}}$}& - & 0.13 & 0.44 & -0.11 & 0.91 \\
\bottomrule
\end{tabular}
}
\caption{\roberta's masked LM loss, before and after \dapt, calculated on samples of held-out documents from each domain. PT denotes a sample from sources similar to \roberta's pretraining corpus.
% See \sect{sec:domain_shift} for definitions of $\Delta\mathcal{L}$ and $\Delta\widetilde{\mathcal{L}}$.
}
\label{tab:masked_lm_study_main_deltaL}
\end{table}


